Few-Shot Spoken Language Understanding via Joint Speech-Text Models

Recent work on speech representation models jointly pre-trained with text has demonstrated the potential of improving speech representations by encoding speech and text in a shared space. In this paper, we leverage such shared representations to address the persistent challenge of limited data availability in spoken language understanding tasks. By employing a pre-trained speech-text model, we find that models fine-tuned on text can be effectively transferred to speech testing data. With as little as 1 hour of labeled speech data, our proposed approach achieves comparable performance on spoken language understanding tasks (specifically, sentiment analysis and named entity recognition) when compared to previous methods using speech-only pre-trained models fine-tuned on 10 times more data. Beyond the proof-of-concept study, we also analyze the latent representations. We find that the bottom layers of speech-text models are largely task-agnostic and align speech and text representations into a shared space, while the top layers are more task-specific.

==> tables/ner_lm.tex <==
% \begin{table}[tbh]
%     \setlength{\tabcolsep}{2pt}
%     \centering
%     \begin{tabular}{l c c c c}
%         \toprule
%         \multirow{2}{*}{Model} & \multicolumn{2}{c}{ Labeled Data
%         } & \multicolumn{2}{c}{F1 Score (\%)} \\
%         \cmidrule(lr){2-3}
%         \cmidrule(lr){4-5}
%         & Speech & Text & NER & NER (Label) \\
%         \midrule
%         \textit{Prior works} \\
%         \hspace{2mm} W2V2-B-LS960 & 14.5 hrs & & 68.1 & \\ 
%         \hspace{2mm} HuBERT-B-LS960 & 14.5 hrs & & 67.8 & \\ 
%         % \hspace{2mm} CMSST & $*$ & full & 38.0 & 49.3 \\
%         \midrule
%         \textit{Baselines} \\
%         \hspace{2mm} SpeechLM-P-B & 14.5 hrs & & 73.0 & 82.6 \\ 
%         \hspace{2mm} SpeechLM-P-B & 14.5 hrs (synth) & & 66.9 & 77.7 \\ 
%         \midrule
%         \textit{Proposed} \\
%         \hspace{2mm} SpeechLM-P-B & & full & 18.1 & 18.4 \\
%         \hspace{2mm} SpeechLM-P-B & 10 mins & full & 51.2 & 59.7 \\ 
%         \hspace{2mm} SpeechLM-P-B & 1 hrs & full & 63.4 & 73.2 \\
%         \bottomrule
%         % \multicolumn{5}{l}{\parbox{\linewidth}{$^*$\scriptsize{CMSST does not use labeled speech data but use speech-transcription pairs of roughly}
%         % \scriptsize{2.5 times of the size of SLUE NER dataset.}}}
%     \end{tabular}
%     \caption{F1 scores of the Named Entity Recognition task on SLUE dev set with LM decoding}
%     \label{tab:NER_lm_results}
% \end{table}

\begin{table*}[ht!]
    \setlength{\tabcolsep}{1.5pt}
    \caption{$F_1$ scores (\%) of the Named Entity Recognition task on the SLUE test set with LM decoding.}
    \footnotesize
    \centering
    \begin{tabular}{l c r r r r r r r r r r}
        \toprule
        \multicolumn{2}{c}{Labeled Data
        } & \multicolumn{5}{c}{$F_1$ (\%)} & \multicolumn{3}{c}{Label-$F_1$ (\%)
        }\\
        \cmidrule(lr){1-2}
        \cmidrule(lr){3-7}
        \cmidrule(lr){8-12}
        Speech & Text & W2V2~\cite{shon2022slue} & HuBERT~\cite{shon2022slue} &  \cmcremove{SPLM}\cmcedit{SpeechLM}-P & \cmcremove{SPLM}\cmcedit{SpeechLM}-H & \cmcremove{SPUT}\cmcedit{SpeechUT} & W2V2~\cite{shon2022slue} & HuBERT~\cite{shon2022slue} & \cmcremove{SPLM}\cmcedit{SpeechLM}-P & \cmcremove{SPLM}\cmcedit{SpeechLM}-H & \cmcremove{SPUT}\cmcedit{SpeechUT} \\
        \midrule
        \textit{Baselines} \\
        % \cmcedit{\hspace{2mm} 1 hr} & - & & & 56.7 & 56.5 & 54.2 & & & 65.9 & 64.2 & 62.8 \\
        % \cmcedit{\hspace{2mm} 3 hrs} & - & & & 67.0 & 66.7 & 66.7 & & & 77.5 & 75.7 & 75.5 \\
        \hspace{2mm} 14.5 hrs & - & 63.4 & 61.9 & \cmcedit{67.1}\cmcremove{73.0} & \cmcedit{67.0}\cmcremove{73.1} & \cmcedit{66.9}\cmcremove{72.8} & 71.7 & 70.3 & \cmcedit{75.8}\cmcremove{81.8} & \cmcedit{76.5}\cmcremove{82.1} & \cmcedit{75.2}\cmcremove{81.8} \\
        \midrule
        \textit{Proposed} \\
        \hspace{2mm} - & full & & & \cmcedit{$^*$8.1}\cmcremove{$^*$9.3} & \cmcedit{$^*$25.7}\cmcremove{$^*$29.4} & \cmcedit{$^*$45.1}\cmcremove{$^*$48.4} & & & \cmcedit{$^*$8.2}\cmcremove{$^*$9.4} & \cmcedit{$^*$30.0}\cmcremove{$^*$33.3} & \cmcedit{$^*$53.9}\cmcremove{$^*$58.3} \\
        \hspace{2mm} 1 hr & full & & & \cmcedit{56.9}\cmcremove{62.5} & \cmcedit{58.7}\cmcremove{63.4} & \cmcedit{58.3}\cmcremove{63.3} & & & \cmcedit{65.9}\cmcremove{71.7} & \cmcedit{67.7}\cmcremove{72.2} & \cmcedit{67.2}\cmcremove{72.4} \\
        % \cmcedit{\hspace{2mm} 2 hrs} & full & & & 68.5 & 67.1 & 67.1 & & & 77.6 & 76.5 & 77.2 \\
        \cmcedit{\hspace{2mm} 3 hrs} & full & & & \cmcedit{62.8}\cmcremove{69.7} & \cmcedit{63.8}\cmcremove{69.2} & \cmcedit{62.6}\cmcremove{69.9} & & & \cmcedit{72.8}\cmcremove{78.8} & \cmcedit{72.9}\cmcremove{78.5} & \cmcedit{72.0}\cmcremove{78.9} \\
        % \cmcedit{\hspace{2mm} 14.5 hrs} & full & & & 72.2 & 72.9 & 73.1 & & & 81.2 & 82.2 & 82.2 \\
        % Speech & Text & W2V2 & HuBERT &  \cmcremove{SPLM}\cmcedit{SpeechLM}-P & \cmcremove{SPLM}\cmcedit{SpeechLM}-H & \cmcremove{SPUT}\cmcedit{SpeechUT} & \cmcremove{SPLM}\cmcedit{SpeechLM}-P & \cmcremove{SPLM}\cmcedit{SpeechLM}-H & \cmcremove{SPUT}\cmcedit{SpeechUT} \\
        % \midrule
        % \textit{Baselines} \\
        % \hspace{2mm} 14.5 hrs & - & 68.1 & 67.8 & 73.0 & 73.1 & 72.8 & 81.8 & 82.1 & 81.8 \\ 
        % \hspace{2mm} 14.5 hrs (syn) & - & & & 58.6 & 61.1 & 59.9 & 70.7 & 72.4 & 71.6 \\ 
        % \midrule
        % \textit{Proposed} \\
        % \hspace{2mm} - & full & & & 9.3 & 29.4 & 48.4 & 9.5 & 33.4 & 58.3 \\
        % \hspace{2mm} 10 mins & full & & & 50.4 & 51.7 & 51.8 & 56.5 & 58.1 & 59.3 \\ 
        % \hspace{2mm} 1 hrs & full & & & 62.5 & 63.4 & 63.3 & 71.7 & 72.2 & 72.4 \\
        \bottomrule
        \multicolumn{10}{l}{\scriptsize$^*$ For text-only fine-tuning, we fine-tune only the top 3 layers of the shared Transformer.}\\
        \multicolumn{10}{l}{\cmc{We need to reduce fontsize to make space for the fullnames of the models (i.e. SpeechLM \& SpeechUT).}}
    \end{tabular}
    \label{tab:NER_lm_results}
    \vspace{-3mm}
\end{table*}

==> tables/ner_nolm.tex <==
% \begin{table}[tbh]
%     \setlength{\tabcolsep}{2pt}
%     \centering
%     \begin{tabular}{l c c c c}
%         \toprule
%         \multirow{2}{*}{Model} & \multicolumn{2}{c}{ Labeled Data
%         } & \multicolumn{2}{c}{F1 Score (\%)} \\
%         \cmidrule(lr){2-3}
%         \cmidrule(lr){4-5}
%         & Speech & Text & NER & NER (Label) \\
%         \midrule
%         \textit{Prior works} \\
%         \hspace{2mm} W2V2-B-LS960 & 14.5 hrs & & 55.0 & \\ 
%         \hspace{2mm} HuBERT-B-LS960 & 14.5 hrs & & 54.5 & \\ 
%         \midrule
%         \textit{Baselines} \\
%         \hspace{2mm} SpeechLM-P-B & 14.5 hrs & & 65.8 & 78.0 \\ 
%         \hspace{2mm} SpeechLM-P-B & 14.5 hrs (synth) & & 59.3 & 75.7 \\ 
%         \midrule
%         \textit{Proposed} \\
%         \hspace{2mm} SpeechLM-P-B & & full & 0.2 & 0.3 \\
%         \hspace{2mm} SpeechLM-P-B & 10 mins & full & 35.4 & 47.7 \\ 
%         \hspace{2mm} SpeechLM-P-B & 1 hrs & full & 52.1 & 67.6 \\
%         \bottomrule
%     \end{tabular}
%     \caption{F1 scores of the Named Entity Recognition task on SLUE dev set without LM decoding. }
%     % Training SpeechLM-P-B model on full set of speech data outperforms the prior works.}
%     \label{tab:NER_nolm_results}
% \end{table}

\begin{table*}[ht!]
    \setlength{\tabcolsep}{1.5pt}
    \caption{$F_1$ scores (\%) of the Named Entity Recognition task on the SLUE test set without LM decoding. Both baselines and proposed approaches show performance comparable to or better than the prior work.}
    \footnotesize
    \centering
    \begin{tabular}{l c r r r r r r r r r r}
        \toprule
        \multicolumn{2}{c}{Labeled Data
        } & \multicolumn{5}{c}{$F_1$ (\%)} & \multicolumn{3}{c}{Label-$F_1$ (\%)
        }\\
        \cmidrule(lr){1-2}
        \cmidrule(lr){3-7}
        \cmidrule(lr){8-12}
        Speech & Text & W2V2~\cite{shon2022slue} & HuBERT~\cite{shon2022slue} &  \cmcremove{SPLM}\cmcedit{SpeechLM}-P & \cmcremove{SPLM}\cmcedit{SpeechLM}-H & \cmcremove{SPUT}\cmcedit{SpeechUT} & W2V2~\cite{shon2022slue} & HuBERT~\cite{shon2022slue} & \cmcremove{SPLM}\cmcedit{SpeechLM}-P & \cmcremove{SPLM}\cmcedit{SpeechLM}-H & \cmcremove{SPUT}\cmcedit{SpeechUT}\\
        \midrule
        \textit{Baselines} \\
        % \cmcedit{\hspace{2mm} 1 hr} & - & & & 43.2 & 40.1 & 36.6 & 58.0 & 54.8 & 51.6 \\
        % \cmcedit{\hspace{2mm} 3 hrs} & - & & & 58.3 & 56.1 & 53.9 & 72.1 & 70.0 & 68.7 \\
        \hspace{2mm} 14.5 hrs & - & 49.6 & 49.8 & \cmcedit{57.9}\cmcremove{64.2} & \cmcedit{57.0}\cmcremove{64.0} & \cmcedit{58.5}\cmcremove{62.9} & 64.0 & 62.9 & \cmcedit{71.8}\cmcremove{76.4} & \cmcedit{72.2}\cmcremove{78.2} & \cmcedit{71.4}\cmcremove{77.2} \\ 
        \hspace{2mm} 14.5 hrs (syn) & - & & & \cmcedit{41.7}\cmcremove{46.4} & \cmcedit{37.4}\cmcremove{41.9} & \cmcedit{34.2}\cmcremove{36.3} & & & \cmcedit{60.9}\cmcremove{64.0} & \cmcedit{58.4}\cmcremove{60.9} & \cmcedit{55.1}\cmcremove{59.6} \\ 
        \midrule
        \textit{Proposed} \\
        \hspace{2mm} - & full & & & \cmcedit{$^*$0.3}\cmcremove{$^*$0.0} & \cmcedit{$^*$1.4}\cmcremove{$^*$1.2} & \cmcedit{$^*$9.7}\cmcremove{$^*$9.7} & & & \cmcedit{$^*$0.4}\cmcremove{$^*$0.2} & \cmcedit{$^*$6.9}\cmcremove{$^*$7.1} & \cmcedit{$^*$31.2}\cmcremove{$^*$32.8} \\
        \hspace{2mm} 10 mins & full & & & \cmcedit{34.2}\cmcremove{35.6} & \cmcedit{31.8}\cmcremove{34.7} & \cmcedit{28.9}\cmcremove{31.5} & & & \cmcedit{45.1}\cmcremove{45.6} & \cmcedit{44.4}\cmcremove{45.8} & \cmcedit{45.3}\cmcremove{46.5} \\ 
        \hspace{2mm} 1 hr & full & & & \cmcedit{46.1}\cmcremove{50.2} & \cmcedit{44.3}\cmcremove{52.0} & \cmcedit{44.2}\cmcremove{47.3} & & & \cmcedit{60.4}\cmcremove{65.1} & \cmcedit{60.1}\cmcremove{65.9} & \cmcedit{61.5}\cmcremove{64.9} \\
        % \cmcedit{\hspace{2mm} 2 hrs} & full & & & 56.7 & 56.9 & 56.0 & & & 70.5 & 71.1 & 70.2 \\
        \cmcedit{\hspace{2mm} 3 hrs} & full & & & \cmcedit{54.1}\cmcremove{60.0} & \cmcedit{52.9}\cmcremove{59.6} & \cmcedit{52.8}\cmcremove{58.2} & & & \cmcedit{68.5}\cmcremove{73.4} & \cmcedit{68.4}\cmcremove{74.9} & \cmcedit{67.8}\cmcremove{73.4} \\
        % \cmcedit{\hspace{2mm} 14.5 hrs} & full & & & 64.5 & 63.3 & 62.5 & & & 77.4 & 77.9 & 76.7 \\
        % \bottomrule
        % Speech & Text & W2V2 & HuBERT &  \cmcremove{SPLM}\cmcedit{SpeechLM}-P & \cmcremove{SPLM}\cmcedit{SpeechLM}-H & \cmcremove{SPUT}\cmcedit{SpeechUT} & \cmcremove{SPLM}\cmcedit{SpeechLM}-P & \cmcremove{SPLM}\cmcedit{SpeechLM}-H & \cmcremove{SPUT}\cmcedit{SpeechUT}\\
        % \midrule
        % \textit{Baselines} \\
        % \hspace{2mm} 14.5 hrs & - & 55.0 & 54.5 & 64.2 & 64.0 & 62.9 & 76.4 & 78.2 & 77.2 \\ 
        % \hspace{2mm} 14.5 hrs (syn) & - & & & 46.4 & 45.9 & 40.3 & 64.0 & 65.4 & 61.8 \\ 
        % \midrule
        % \textit{Proposed} \\
        % \hspace{2mm} - & full & & & 0.2 & 1.2* & 14.8 & 0.3 & 9.3 & 38.3 \\
        % \hspace{2mm} 10 mins & full & & & 35.6 & 34.7 & 31.5 & 45.6 & 45.8 & 46.5 \\ 
        % \hspace{2mm} 1 hrs & full & & & 50.2 & 52.0 & 47.3 & 65.1 & 65.9 & 64.9 \\
        \bottomrule
        \multicolumn{10}{l}{\scriptsize$^*$ For text-only fine-tuning, we fine-tune only the top 3 layers of the shared Transformer. Related details can be found in Sec. \ref{ssec:frozen}.}\\
        \multicolumn{10}{l}{\cmc{We need to reduce fontsize to make space for the fullnames of the models (i.e. SpeechLM \& SpeechUT).}}
    \end{tabular}
    \label{tab:NER_nolm_results}
    \vspace{-6mm}
\end{table*}
